SPP: Sparsity-Preserved Parameter-Efficient Fine-Tuning for Large Language Models

Large Language Models (LLMs) have become pivotal in advancing the field of artificial intelligence, yet their immense sizes pose significant challenges for both fine-tuning and deployment. Current post-training pruning methods, while reducing the sizes of LLMs, often fail to maintain their original performance. To address these challenges, this paper introduces SPP, a Sparsity-Preserved Parameter-efficient fine-tuning method. Different from existing post-training pruning approaches that struggle with performance retention, SPP proposes to employ lightweight learnable column and row matrices to optimize sparse LLM weights, keeping the structure and sparsity of pruned pre-trained models intact. By element-wise multiplication and residual addition, SPP ensures the consistency of model sparsity pattern and ratio during both training and weight-merging processes. We demonstrate the effectiveness of SPP by applying it to the LLaMA and LLaMA-2 model families with recent post-training pruning methods. Our results show that SPP significantly enhances the performance of models with different sparsity patterns (i.e. unstructured and N:M sparsity), especially for those with high sparsity ratios (e.g. 75%), making it a promising solution for the efficient fine-tuning of sparse LLMs. Code will be made available at https://github.com/Lucky-Lance/SPP.

==> icml2024/table_result/ppl.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[h!]\fontsize{8.5}{9}\selectfont
\centering
\resizebox{\textwidth}{!}{%
% \begin{tabular}{ccccccccc}
\begin{tabular*}{\hsize}{@{}@{\extracolsep{\fill}}ccccccccc@{}}\midrule
% \begin{tabular}{ccccccccc}
               &                  & \multicolumn{4}{c}{\textbf{LLaMA}} & \multicolumn{3}{c}{\textbf{LLaMA - 2}}       \\\midrule
\textbf{Algorithm}      & \textbf{Sparsity}         & \textbf{7B}    & \textbf{13B}   & \textbf{30B}   & \textbf{65B}   & \textbf{7B}        & \textbf{13B}   & \textbf{70B}   \\\midrule
N/A            & Dense            & 5.68 & 5.09  & 4.10  & 3.53  & 5.12      & 4.57   & 3.12  \\\midrule
SparseGPT      & Unstructured 50\% & 7.21  & 6.21  & 5.32  & 4.60  & 6.52      & 5.62  & 3.99  \\
SparseGPT\textbf{+Ours} & Unstructured 50\% & 7.27  & 6.09  & 5.36  & 4.59 & 6.35      & 5.42  & 3.99   \\
SparseGPT      & 2:4            & 10.87  & 9.09  & 7.20  & 6.20  & 10.06      & 8.12  & 5.37  \\
SparseGPT\textbf{+Ours} & 2:4            & 8.71  & 7.11  & 6.20  & 6.12   & 7.66      & 6.41  & 5.36  \\\midrule
Wanda          & Unstructured 50\% & 7.26    & 6.15  & 5.25  & 4.60  & 6.46       & 5.58  & 3.97  \\
Wanda\textbf{+Ours}     & Unstructured 50\% & 7.28  & 6.10  & 5.26  & 4.59  & 6.26      & 5.41  & 3.97  \\
Wanda          & 2:4            & 11.53  & 9.57  & 6.90  & 6.24  & 11.32      & 8.37  & 5.20  \\
Wanda\textbf{+Ours}     & 2:4            & 8.72  & 7.20  & 6.20  & 5.90  & 7.78      & 6.49  & 5.07 \\\midrule
\end{tabular*}%
}
\caption{Wikitext PPL~\cite{merity2016pointer} comparison of 50\% sparsity models before andafter SPP fine-tuning. After training, the PPL of all models with 2:4 structured sparsity decreased, and the PPL of most unstructured 50\% sparsity models decreased.}
\label{tab:ppl_cmp}
\end{table*}


==> sec/x_icml.tex <==
\section{Related Works}

\subsection{xxx}

Submission to ICML 2024 will be entirely electronic, via a web site
(not email). Information about the submission process and \LaTeX\ templates
are available on the conference web site at:
\begin{center}
\textbf{\texttt{http://icml.cc/}}
\end{center}

The guidelines below will be enforced for initial submissions and
camera-ready copies. Here is a brief summary:
\begin{itemize}
\item Submissions must be in PDF\@. 
\item \textbf{New to this year}: If your paper has appendices, submit the appendix together with the main body and the references \textbf{as a single file}. Reviewers will not look for appendices as a separate PDF file. So if you submit such an extra file, reviewers will very likely miss it.
\item Page limit: The main body of the paper has to be fitted to 8 pages, excluding references and appendices; the space for the latter two is not limited. For the final version of the paper, authors can add one extra page to the main body.
\item \textbf{Do not include author information or acknowledgements} in your
    initial submission.
\item Your paper should be in \textbf{10 point Times font}.
\item Make sure your PDF file only uses Type-1 fonts.
\item Place figure captions \emph{under} the figure (and omit titles from inside
    the graphic file itself). Place table captions \emph{over} the table.
\item References must include page numbers whenever possible and be as complete
    as possible. Place multiple citations in chronological order.
\item Do not alter the style template; in particular, do not compress the paper
    format by reducing the vertical spaces.
\item Keep your abstract brief and self-contained, one paragraph and roughly
    4--6 sentences. Gross violations will require correction at the
    camera-ready phase. The title should have content words capitalized.
\end{itemize}

\subsection{Submitting Papers}

\textbf{Paper Deadline:} The deadline for paper submission that is
advertised on the conference website is strict. If your full,
anonymized, submission does not reach us on time, it will not be
considered for publication. 

\textbf{Anonymous Submission:} ICML uses double-blind review: no identifying
author information may appear on the title page or in the paper
itself. \cref{author info} gives further details.

\textbf{Simultaneous Submission:} ICML will not accept any paper which,
at the time of submission, is under review for another conference or
has already been published. This policy also applies to papers that
overlap substantially in technical content with conference papers
under review or previously published. ICML submissions must not be
submitted to other conferences and journals during ICML's review
period.
%Authors may submit to ICML substantially different versions of journal papers
%that are currently under review by the journal, but not yet accepted
%at the time of submission.
Informal publications, such as technical
reports or papers in workshop proceedings which do not appear in
print, do not fall under these restrictions.

\medskip

Authors must provide their manuscripts in \textbf{PDF} format.
Furthermore, please make sure that files contain only embedded Type-1 fonts
(e.g.,~using the program \texttt{pdffonts} in linux or using
File/DocumentProperties/Fonts in Acrobat). Other fonts (like Type-3)
might come from graphics files imported into the document.

Authors using \textbf{Word} must convert their document to PDF\@. Most
of the latest versions of Word have the facility to do this
automatically. Submissions will not be accepted in Word format or any
format other than PDF\@. Really. We're not joking. Don't send Word.

Those who use \textbf{\LaTeX} should avoid including Type-3 fonts.
Those using \texttt{latex} and \texttt{dvips} may need the following
two commands:

{\footnotesize
\begin{verbatim}
dvips -Ppdf -tletter -G0 -o paper.ps paper.dvi
ps2pdf paper.ps
\end{verbatim}}
It is a zero following the ``-G'', which tells dvips to use
the config.pdf file. Newer \TeX\ distributions don't always need this
option.

Using \texttt{pdflatex} rather than \texttt{latex}, often gives better
results. This program avoids the Type-3 font problem, and supports more
advanced features in the \texttt{microtype} package.

\textbf{Graphics files} should be a reasonable size, and included from
an appropriate format. Use vector formats (.eps/.pdf) for plots,
lossless bitmap formats (.png) for raster graphics with sharp lines, and
jpeg for photo-like images.

The style file uses the \texttt{hyperref} package to make clickable
links in documents. If this causes problems for you, add
\texttt{nohyperref} as one of the options to the \texttt{icml2024}
usepackage statement.


\subsection{Submitting Final Camera-Ready Copy}

The final versions of papers accepted for publication should follow the
same format and naming convention as initial submissions, except that
author information (names and affiliations) should be given. See
\cref{final author} for formatting instructions.

The footnote, ``Preliminary work. Under review by the International
Conference on Machine Learning (ICML). Do not distribute.'' must be
modified to ``\textit{Proceedings of the
$\mathit{41}^{st}$ International Conference on Machine Learning},
Vienna, Austria, PMLR 235, 2024.
Copyright 2024 by the author(s).''

For those using the \textbf{\LaTeX} style file, this change (and others) is
handled automatically by simply changing
$\mathtt{\backslash usepackage\{icml2024\}}$ to
$$\mathtt{\backslash usepackage[accepted]\{icml2024\}}$$
Authors using \textbf{Word} must edit the
footnote on the first page of the document themselves.

Camera-ready copies should have the title of the paper as running head
on each page except the first one. The running title consists of a
single line centered above a horizontal rule which is $1$~point thick.
The running head should be centered, bold and in $9$~point type. The
rule should be $10$~points above the main text. For those using the
\textbf{\LaTeX} style file, the original title is automatically set as running
head using the \texttt{fancyhdr} package which is included in the ICML
2024 style file package. In case that the original title exceeds the
size restrictions, a shorter form can be supplied by using

\verb|\icmltitlerunning{...}|

just before $\mathtt{\backslash begin\{document\}}$.
Authors using \textbf{Word} must edit the header of the document themselves.

\section{Format of the Paper}

All submissions must follow the specified format.

\subsection{Dimensions}




The text of the paper should be formatted in two columns, with an
overall width of 6.75~inches, height of 9.0~inches, and 0.25~inches
between the columns. The left margin should be 0.75~inches and the top
margin 1.0~inch (2.54~cm). The right and bottom margins will depend on
whether you print on US letter or A4 paper, but all final versions
must be produced for US letter size.
Do not write anything on the margins.

The paper body should be set in 10~point type with a vertical spacing
of 11~points. Please use Times typeface throughout the text.

\subsection{Title}

The paper title should be set in 14~point bold type and centered
between two horizontal rules that are 1~point thick, with 1.0~inch
between the top rule and the top edge of the page. Capitalize the
first letter of content words and put the rest of the title in lower
case.

\subsection{Author Information for Submission}
\label{author info}

ICML uses double-blind review, so author information must not appear. If
you are using \LaTeX\/ and the \texttt{icml2024.sty} file, use
\verb+\icmlauthor{...}+ to specify authors and \verb+\icmlaffiliation{...}+ to specify affiliations. (Read the TeX code used to produce this document for an example usage.) The author information
will not be printed unless \texttt{accepted} is passed as an argument to the
style file.
Submissions that include the author information will not
be reviewed.

\subsubsection{Self-Citations}

If you are citing published papers for which you are an author, refer
to yourself in the third person. In particular, do not use phrases
that reveal your identity (e.g., ``in previous work \cite{langley00}, we
have shown \ldots'').

Do not anonymize citations in the reference section. The only exception are manuscripts that are
not yet published (e.g., under submission). If you choose to refer to
such unpublished manuscripts \cite{anonymous}, anonymized copies have
to be submitted
as Supplementary Material via OpenReview\@. However, keep in mind that an ICML
paper should be self contained and should contain sufficient detail
for the reviewers to evaluate the work. In particular, reviewers are
not required to look at the Supplementary Material when writing their
review (they are not required to look at more than the first $8$ pages of the submitted document).

\subsubsection{Camera-Ready Author Information}
\label{final author}

If a paper is accepted, a final camera-ready copy must be prepared.
%
For camera-ready papers, author information should start 0.3~inches below the
bottom rule surrounding the title. The authors' names should appear in 10~point
bold type, in a row, separated by white space, and centered. Author names should
not be broken across lines. Unbolded superscripted numbers, starting 1, should
be used to refer to affiliations.

Affiliations should be numbered in the order of appearance. A single footnote
block of text should be used to list all the affiliations. (Academic
affiliations should list Department, University, City, State/Region, Country.
Similarly for industrial affiliations.)

Each distinct affiliations should be listed once. If an author has multiple
affiliations, multiple superscripts should be placed after the name, separated
by thin spaces. If the authors would like to highlight equal contribution by
multiple first authors, those authors should have an asterisk placed after their
name in superscript, and the term ``\textsuperscript{*}Equal contribution"
should be placed in the footnote block ahead of the list of affiliations. A
list of corresponding authors and their emails (in the format Full Name
\textless{}email@domain.com\textgreater{}) can follow the list of affiliations.
Ideally only one or two names should be listed.

A sample file with author names is included in the ICML2024 style file
package. Turn on the \texttt{[accepted]} option to the stylefile to
see the names rendered. All of the guidelines above are implemented
by the \LaTeX\ style file.

\subsection{Abstract}

The paper abstract should begin in the left column, 0.4~inches below the final
address. The heading `Abstract' should be centered, bold, and in 11~point type.
The abstract body should use 10~point type, with a vertical spacing of
11~points, and should be indented 0.25~inches more than normal on left-hand and
right-hand margins. Insert 0.4~inches of blank space after the body. Keep your
abstract brief and self-contained, limiting it to one paragraph and roughly 4--6
sentences. Gross violations will require correction at the camera-ready phase.

\subsection{Partitioning the Text}

You should organize your paper into sections and paragraphs to help
readers place a structure on the material and understand its
contributions.

\subsubsection{Sections and Subsections}

Section headings should be numbered, flush left, and set in 11~pt bold
type with the content words capitalized. Leave 0.25~inches of space
before the heading and 0.15~inches after the heading.

Similarly, subsection headings should be numbered, flush left, and set
in 10~pt bold type with the content words capitalized. Leave
0.2~inches of space before the heading and 0.13~inches afterward.

Finally, subsubsection headings should be numbered, flush left, and
set in 10~pt small caps with the content words capitalized. Leave
0.18~inches of space before the heading and 0.1~inches after the
heading.

Please use no more than three levels of headings.

\subsubsection{Paragraphs and Footnotes}

Within each section or subsection, you should further partition the
paper into paragraphs. Do not indent the first line of a given
paragraph, but insert a blank line between succeeding ones.

You can use footnotes\footnote{Footnotes
should be complete sentences.} to provide readers with additional
information about a topic without interrupting the flow of the paper.
Indicate footnotes with a number in the text where the point is most
relevant. Place the footnote in 9~point type at the bottom of the
column in which it appears. Precede the first footnote in a column
with a horizontal rule of 0.8~inches.\footnote{Multiple footnotes can
appear in each column, in the same order as they appear in the text,
but spread them across columns and pages if possible.}

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{icml_numpapers}}
\caption{Historical locations and number of accepted papers for International
Machine Learning Conferences (ICML 1993 -- ICML 2008) and International
Workshops on Machine Learning (ML 1988 -- ML 1992). At the time this figure was
produced, the number of accepted papers for ICML 2008 was unknown and instead
estimated.}
\label{icml-historical}
\end{center}
\vskip -0.2in
\end{figure}

\subsection{Figures}

You may want to include figures in the paper to illustrate
your approach and results. Such artwork should be centered,
legible, and separated from the text. Lines should be dark and at
least 0.5~points thick for purposes of reproduction, and text should
not appear on a gray background.

Label all distinct components of each figure. If the figure takes the
form of a graph, then give a name for each axis and include a legend
that briefly describes each curve. Do not include a title inside the
figure; instead, the caption should serve this function.

Number figures sequentially, placing the figure number and caption
\emph{after} the graphics, with at least 0.1~inches of space before
the caption and 0.1~inches after it, as in
\cref{icml-historical}. The figure caption should be set in
9~point type and centered unless it runs two or more lines, in which
case it should be flush left. You may float figures to the top or
bottom of a column, and you may set wide figures across both columns
(use the environment \texttt{figure*} in \LaTeX). Always place
two-column figures at the top or bottom of the page.

\subsection{Algorithms}

If you are using \LaTeX, please use the ``algorithm'' and ``algorithmic''
environments to format pseudocode. These require
the corresponding stylefiles, algorithm.sty and
algorithmic.sty, which are supplied with this package.
\cref{alg:example} shows an example.

\begin{algorithm}[tb]
   \caption{Bubble Sort}
   \label{alg:example}
\begin{algorithmic}
   \STATE {\bfseries Input:} data $x_i$, size $m$
   \REPEAT
   \STATE Initialize $noChange = true$.
   \FOR{$i=1$ {\bfseries to} $m-1$}
   \IF{$x_i > x_{i+1}$}
   \STATE Swap $x_i$ and $x_{i+1}$
   \STATE $noChange = false$
   \ENDIF
   \ENDFOR
   \UNTIL{$noChange$ is $true$}
\end{algorithmic}
\end{algorithm}

\subsection{Tables}

You may also want to include tables that summarize material. Like
figures, these should be centered, legible, and numbered consecutively.
However, place the title \emph{above} the table with at least
0.1~inches of space before the title and the same after it, as in
\cref{sample-table}. The table title should be set in 9~point
type and centered unless it runs two or more lines, in which case it
should be flush left.

% Note use of \abovespace and \belowspace to get reasonable spacing
% above and below tabular lines.

\begin{table}[t]
\caption{Classification accuracies for naive Bayes and flexible
Bayes on various data sets.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Data set & Naive & Flexible & Better? \\
\midrule
Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

Tables contain textual material, whereas figures contain graphical material.
Specify the contents of each row and column in the table's topmost
row. Again, you may float tables to a column's top or bottom, and set
wide tables across both columns. Place two-column tables at the
top or bottom of the page.

\subsection{Theorems and such}
The preferred way is to number definitions, propositions, lemmas, etc. consecutively, within sections, as shown below.
\begin{definition}
\label{def:inj}
A function $f:X \to Y$ is injective if for any $x,y\in X$ different, $f(x)\ne f(y)$.
\end{definition}
Using \cref{def:inj} we immediate get the following result:
\begin{proposition}
If $f$ is injective mapping a set $X$ to another set $Y$, 
the cardinality of $Y$ is at least as large as that of $X$
\end{proposition}
\begin{proof} 
Left as an exercise to the reader. 
\end{proof}
\cref{lem:usefullemma} stated next will prove to be useful.
\begin{lemma}
\label{lem:usefullemma}
For any $f:X \to Y$ and $g:Y\to Z$ injective functions, $f \circ g$ is injective.
\end{lemma}
\begin{theorem}
\label{thm:bigtheorem}
If $f:X\to Y$ is bijective, the cardinality of $X$ and $Y$ are the same.
\end{theorem}
An easy corollary of \cref{thm:bigtheorem} is the following:
\begin{corollary}
If $f:X\to Y$ is bijective, 
the cardinality of $X$ is at least as large as that of $Y$.
\end{corollary}
\begin{assumption}
The set $X$ is finite.
\label{ass:xfinite}
\end{assumption}
\begin{remark}
According to some, it is only the finite case (cf. \cref{ass:xfinite}) that is interesting.
\end{remark}
%restatable

\subsection{Citations and References}

Please use APA reference format regardless of your formatter
or word processor. If you rely on the \LaTeX\/ bibliographic
facility, use \texttt{natbib.sty} and \texttt{icml2024.bst}
included in the style-file package to obtain this format.

Citations within the text should include the authors' last names and
year. If the authors' names are included in the sentence, place only
the year in parentheses, for example when referencing Arthur Samuel's
pioneering work \yrcite{Samuel59}. Otherwise place the entire
reference in parentheses with the authors and year separated by a
comma \cite{Samuel59}. List multiple references separated by
semicolons \cite{kearns89,Samuel59,mitchell80}. Use the `et~al.'
construct only for citations with three or more authors or after
listing all authors to a publication in an earlier reference \cite{MachineLearningI}.

Authors should cite their own work in the third person
in the initial version of their paper submitted for blind review.
Please refer to \cref{author info} for detailed instructions on how to
cite your own papers.

Use an unnumbered first-level section heading for the references, and use a
hanging indent style, with the first line of the reference flush against the
left margin and subsequent lines indented by 10 points. The references at the
end of this document give examples for journal articles \cite{Samuel59},
conference publications \cite{langley00}, book chapters \cite{Newell81}, books
\cite{DudaHart2nd}, edited volumes \cite{MachineLearningI}, technical reports
\cite{mitchell80}, and dissertations \cite{kearns89}.

Alphabetize references by the surnames of the first authors, with
single author entries preceding multiple author entries. Order
references for the same authors by year of publication, with the
earliest first. Make sure that each reference includes all relevant
information (e.g., page numbers).

Please put some effort into making references complete, presentable, and
consistent, e.g. use the actual current name of authors.
If using bibtex, please protect capital letters of names and
abbreviations in titles, for example, use \{B\}ayesian or \{L\}ipschitz
in your .bib file.

\section*{Accessibility}
Authors are kindly asked to make their submissions as accessible as possible for everyone including people with disabilities and sensory or neurological differences.
Tips of how to achieve this and what to pay attention to will be provided on the conference website \url{http://icml.cc/}.

\section*{Software and Data}

If a paper is accepted, we strongly encourage the publication of software and data with the
camera-ready version of the paper whenever appropriate. This can be
done by including a URL in the camera-ready copy. However, \textbf{do not}
include URLs that reveal your institution or identity in your
submission for review. Instead, provide an anonymous URL or upload
the material as ``Supplementary Material'' into the OpenReview reviewing
system. Note that reviewers are not required to look at this material
when writing their review.

% Acknowledgements should only appear in the accepted version.
\section*{Acknowledgements}

\textbf{Do not} include acknowledgements in the initial version of
the paper submitted for blind review.

If a paper is accepted, the final camera-ready version can (and
probably should) include acknowledgements. In this case, please
place such acknowledgements in an unnumbered section at the
end of the paper. Typically, this will include thanks to reviewers
who gave useful comments, to colleagues who contributed to the ideas,
and to funding agencies and corporate sponsors that provided financial
support.

==> table_result/DSnoT.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[t]\huge
\centering
\vspace{-0.1em}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{clccc}
\midrule
{ \textbf{LLaMA}} &
  { \textbf{Method}} &
  { \textbf{Sparsity}} &
  { \textbf{LM-eval}} & {\textbf{PPL ($\mathbf{\downarrow}$)}} \\ \midrule
 &
   { Wanda} &
  { Unstructured 75\%} &
  32.14& {1285.24} \\ % \cmidrule{2-4} 
&
  { Wanda+DS$\oslash$T} &
  { Unstructured 75\%} &
  32.23 & { 646.40} \\ % \cmidrule{2-4} 
 &
  { Wanda\textbf{+SPP}} &
  { Unstructured 75\%} &
  \textbf{41.71}&\textbf{ 21.80} \\ \cmidrule{2-5}
 &
    { Wanda} &
  { 2:8} &
  32.53& { 3284.43} \\ % \cmidrule{2-4} 
&
  { Wanda+DS$\oslash$T} &
  { 2:8} &
  31.57 & { 2742.98} \\  
\multirow{-6}{*}{{ \textbf{7B}}} &
  { Wanda\textbf{+SPP}} &
  { 2:8} &
  \textbf{38.61}& \textbf{ 42.07 } \\ \midrule
 &
   { Wanda} &
  { Unstructured 75\%} &
  39.21& { 149.63} \\
  &
  { Wanda+DS$\oslash$T} &
  { Unstructured 75\%} &
  37.77 & { 184.51} \\ % \cmidrule{2-4} 
 &
  { Wanda\textbf{+SPP}} &
  { Unstructured 75\%} &
  \textbf{50.33}& \textbf{ 10.89} \\ \cmidrule{2-5} 
 &
   { Wanda} &
  { 2:8} &
  35.12& { 1057.58} \\ &
  { Wanda+DS$\oslash$T} &
  { 2:8} &
32.81 & 903.17 \\ % \cmidrule{2-4} 
\multirow{-6}{*}{{ \textbf{30B}}} &
  { Wanda\textbf{+SPP}} &
  { 2:8} &
  \textbf{43.09} & \textbf{19.83} \\ \bottomrule
\end{tabular}%
}
\vspace{-0.3em}
\caption{Comparison for pruning LLaMA model family at 75\% sparsity. We provide average accuracies of 7 zero-shot tasks together with WikiText perplexity~\cite{merity2016pointer}. SPP achieves far better results than the other two post-training pruning methods.}
\label{tab:compare_dsnot}
\vspace{-1.2em}
\end{table}


==> table_result/ablation_study.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t]\huge
\centering
\vspace{-0.1em}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccccc}
\midrule
\textbf{Method} & \textbf{Sparsity}& \textbf{Zero-init} & \textbf{$\W_\beta$} & \textbf{$r$} & \textbf{LM-eval} \\ \midrule
\multirow{10}{*}{{\makecell{Wanda\textbf{+SPP}}}} & \multirow{5}{*}{2:4} & \checkmark & \checkmark & 4 & 54.04 \\ %\cmidrule{3-6} 
 & & \checkmark & \checkmark & 8 & 54.87 \\ %\cmidrule{3-6} 
 & & \checkmark & & 16 & 54.52  \\ %\cmidrule{3-6} 
 & & &\checkmark & 16 & 53.52 \\ % \cmidrule{2-6} 
 & & \checkmark & \checkmark & 16 & \textbf{55.42} \\ \cmidrule{2-6} 
 & \multirow{5}{*}{\makecell{Unstructured 50\%}} & \checkmark &\checkmark & 4 & 57.86 \\ %\cmidrule{3-6} 
 & & \checkmark & \checkmark & 8 & 56.39 \\ %\cmidrule{3-6} 
 & & \checkmark & & 16 & 57.81\\ %\cmidrule{3-6} 
 & & &\checkmark & 16 & 57.59 \\ % \cmidrule{2-6} 
 & & \checkmark & \checkmark & 16 & \textbf{58.13}  \\ \midrule
\multirow{10}{*}{{\makecell{SparseGPT\textbf{+SPP}}}} & \multirow{5}{*}{2:4} & \checkmark & \checkmark& 4 & \textbf{54.82} \\ %\cmidrule{3-6} 
 & & \checkmark & \checkmark & 8 & 54.24\\ %\cmidrule{3-6} 
 & & \checkmark & & 16 & {54.62}\\ %\cmidrule{3-6} 
 & & &\checkmark & 16 & 54.01 \\ % \cmidrule{2-6} 
 & & \checkmark & \checkmark & 16 & 54.60\\ \cmidrule{2-6} 
 & \multirow{5}{*}{{\makecell{Unstructured 50\%}}} & \checkmark & \checkmark & 4 & 57.58 \\ %\cmidrule{3-6} 
 & & \checkmark & \checkmark & 8 & 57.32 \\ %\cmidrule{3-6} 
 & & \checkmark & & 16 & 57.66 \\ %\cmidrule{3-6} 
 & & &\checkmark & 16 & 57.12 \\ % \cmidrule{2-6} 
 & & \checkmark & \checkmark & 16 & \textbf{58.43}  \\ \midrule
\end{tabular}%
}
\vspace{-0.2em}
\caption{Ablation studies on LLaMA-7B. We investigate the utility of zero-initialization of weights, evaluate the influence of parameter $\W_\beta$, as well as test the performance of SPP-trained models for different values of $r$. Training with zero-init weights, $\W_\beta$, and using $r=16$ get the overall best results in our experiments.}
\label{tab:ablation_study}
\vspace{-0.8em}
\end{table}


==> table_result/few_shot_llama1_llama2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[t]\fontsize{8.5}{9}\selectfont
\centering
\resizebox{\textwidth}{!}{%
% \begin{tabular}{ccccccccc}
\begin{tabular*}{\hsize}{@{}@{\extracolsep{\fill}}lcccccccc@{}}\midrule
% \begin{tabular}{ccccccccc}
               &                  & \multicolumn{4}{c}{\textbf{LLaMA}} & \multicolumn{3}{c}{\textbf{LLaMA-2}}       \\\midrule
\textbf{Method}      & \textbf{Sparsity}         & 7B    & 13B   & 30B   & 65B   & {7B}        & {13B}   & {70B}   \\\midrule
None            & Dense            & 35.64 & 47.63 & 58.58 & 63.78 & 46.56     & 55.30  & 69.56 \\\midrule
SparseGPT      & Unstructured 50\% & \gc{32.19} & \gc{40.44} & \gc{52.62} & \gc{59.37} & \gc{36.41}     & \gc{47.47} & \gc{65.57} \\
SparseGPT\textbf{+SPP} & Unstructured 50\% & 30.77 & 43.91 & 54.73 & 59.38 & 39.78     & 48.31 & 65.60  \\\midrule
SparseGPT      & 2:4            & \gc{28.24} & \gc{32.31} & \gc{43.79} & \gc{49.79} & \gc{29.16}     & \gc{38.41} & \gc{57.66} \\
SparseGPT\textbf{+SPP} & 2:4            & 27.81 & 37.55 & 49.01 & 49.50  & 33.28     & 45.63 & 57.85 \\\midrule
Wanda          & Unstructured 50\% & \gc{31.50}  & \gc{39.43} & \gc{52.84} & \gc{58.75} & \gc{34.20}      & \gc{47.78} & \gc{64.45} \\
Wanda\textbf{+SPP}     & Unstructured 50\% & 31.74 & 43.34 & 53.89 & 59.02 & 38.08     & 48.97 & 64.39 \\\midrule
Wanda          & 2:4            & \gc{27.14} & \gc{31.26} & \gc{41.36} & \gc{45.68} & \gc{28.33}     & \gc{35.16} & \gc{56.86} \\
Wanda\textbf{+SPP}     & 2:4            & 28.56 & 35.73 & 46.19 & 47.67 & 30.47     & 42.79 & 57.98\\\midrule
\end{tabular*}%
}
% \vspace{-1em}
\caption{5-shot evaluation of MMLU~\cite{hendrycks2021ethics,hendryckstest2021}, with LLaMA and LLaMA-2 model families trained on Alpaca~\cite{taori2023alpaca} dataset. The performances of sparse models are improved after instruction fine-tuning.}
\label{tab:few_shot_llama1_llama2}
% \vspace{-0.5em}
\end{table*}


==> table_result/high_sparsity.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccccc}
\midrule
\textbf{LLaMA} &
  \textbf{Method} &
  \textbf{Sparsity} &
  \textbf{BoolQ} &
  \textbf{RTE} &
  \textbf{HellaSwag} &
  \textbf{WinoGrande} &
  \textbf{ARC-e} &
  \textbf{ARC-c} &
  \textbf{OBQA} &
  \textbf{Average} \\ \midrule
\multirow{4.5}{*}{\textbf{7B}}
                              & Wanda+LoRA*  & Unstructured 75\%  & 62.39 & 53.07 & 31.81 & 52.64 & 38.22 & 21.08 & 14.60 & 39.11 \\
                              & Wanda\textbf{+SPP} & Unstructured 75\%   & 60.67 & 56.32 & 35.06 & 52.64 & 47.05 & 22.44 & 17.80 & \textbf{41.71} \\ 
 \cmidrule{2-11} 
                               & Wanda+LoRA*  & 2:8               & 61.47 & 53.07 & 29.18 & 53.12 & 34.68 & 20.22 & 14.60 & 38.05 \\
                              & Wanda\textbf{+SPP} & 2:8         & 54.50 & 59.21 & 31.29 & 52.09 & 37.46 & 19.11 & 16.60 & \textbf{38.61} \\ 
 \midrule
\multirow{4.5}{*}{\textbf{30B}}
                              & Wanda+LoRA*  & Unstructured 75\%   & 65.08 & 55.60 & 44.35 & 62.27 & 60.69 & 29.18 & 23.00 & 48.60 \\
                              & Wanda\textbf{+SPP} & Unstructured 75\%   & 67.95 & 54.15 & 47.28 & 62.51 & 63.68 & 30.72 & 26.00 & \textbf{50.33} \\  \cmidrule{2-11} 
                              & Wanda+LoRA*  & 2:8                & 62.17 & 52.71 & 35.96 & 54.30 & 48.48 & 23.21 & 16.20 & 41.86 \\
                              & Wanda\textbf{+SPP} & 2:8                & 62.05 & 54.87 & 38.17 & 55.09 & 49.62 & 23.63 & 18.20 & \textbf{43.09} \\  \midrule
\end{tabular}%
}
% \vspace{-0.5em}
\caption{Zero-shot evaluation of 7 different tasks from EleutherAI LM Harness~\cite{gao2021framework} with 75\% sparsity. We compare SPP with sparse models after LoRA training by applying the dense trained model with the original Wanda pruning masks. SPP achieves overall higher zero-shot performances than LoRA. (*) denotes sparse models obtained from applying Wanda pruning masks after LoRA training.}
\label{tab:high_sparsity}
% \vspace{-0.5em}
\end{table*}


==> table_result/more_abla.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[h!]
\centering
\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{ccccc}
\midrule
{\color[HTML]{000000} \textbf{Method}} &
  {\color[HTML]{000000} \textbf{Sparsity}} &
  {\color[HTML]{000000} \textbf{Zero-init $\W_\alpha$}} &
  {\color[HTML]{000000} \textbf{Zero-init $\W_\beta$}} &
  {\color[HTML]{000000} \textbf{LM-eval}} \\ \midrule
{\color[HTML]{000000} } &
  {\color[HTML]{000000} } &
  {\color[HTML]{000000} } &
  {\color[HTML]{000000} } &
  {\color[HTML]{000000} 53.52} \\ % \cmidrule{3-5} 
{\color[HTML]{000000} } &
  {\color[HTML]{000000} } &
  {\color[HTML]{000000} \checkmark} &
  {\color[HTML]{000000} } &
  {\color[HTML]{000000} \textbf{56.16}} \\ % \cmidrule{3-5} 
{\color[HTML]{000000} } &
  \multirow{-3}{*}{{\color[HTML]{000000} 2:4}} &
  {\color[HTML]{000000} } &
  {\color[HTML]{000000} \checkmark} &
  {\color[HTML]{000000} 55.42} \\ \cmidrule{2-5} 
{\color[HTML]{000000} } &
  {\color[HTML]{000000} } &
  {\color[HTML]{000000} } &
  {\color[HTML]{000000} } &
  {\color[HTML]{000000} 57.59} \\ % \cmidrule{3-5} 
{\color[HTML]{000000} } &
  {\color[HTML]{000000} } &
  {\color[HTML]{000000} \checkmark} &
  {\color[HTML]{000000} } &
  {\color[HTML]{000000} 57.09} \\ % \cmidrule{3-5} 
\multirow{-6}{*}{{\color[HTML]{000000} {Wanda+\textbf{SPP}}}} &
  \multirow{-3}{*}{{\color[HTML]{000000} Unstructured 50\%}} &
  {\color[HTML]{000000} } &
  {\color[HTML]{000000} \checkmark} &
  {\color[HTML]{000000} \textbf{58.13}} \\ \midrule
{\color[HTML]{000000} } &
  {\color[HTML]{000000} } &
  {\color[HTML]{000000} } &
  {\color[HTML]{000000} } &
  {\color[HTML]{000000} 54.01} \\ % \cmidrule{3-5} 
{\color[HTML]{000000} } &
  {\color[HTML]{000000} } &
  {\color[HTML]{000000} \checkmark} &
  {\color[HTML]{000000} } &
  {\color[HTML]{000000} 53.95} \\ % \cmidrule{3-5} 
{\color[HTML]{000000} } &
  \multirow{-3}{*}{{\color[HTML]{000000} 2:4}} &
  {\color[HTML]{000000} } &
  {\color[HTML]{000000} \checkmark} &
  {\color[HTML]{000000} \textbf{54.60}} \\ \cmidrule{2-5} 
{\color[HTML]{000000} } &
  {\color[HTML]{000000} } &
  {\color[HTML]{000000} } &
  {\color[HTML]{000000} } &
  {\color[HTML]{000000} 57.12} \\ % \cmidrule{3-5} 
{\color[HTML]{000000} } &
  {\color[HTML]{000000} } &
  {\color[HTML]{000000} \checkmark} &
  {\color[HTML]{000000} } &
  {\color[HTML]{000000} 57.59} \\ % \cmidrule{3-5} 
\multirow{-6}{*}{{\color[HTML]{000000} {SparseGPT+\textbf{SPP}}}} &
  \multirow{-3}{*}{{\color[HTML]{000000} Unstructured 50\%}} &
  {\color[HTML]{000000} } &
  {\color[HTML]{000000} \checkmark} &
  {\color[HTML]{000000} \textbf{58.43}} \\ \midrule
\end{tabular}%
}
\caption{More ablation studies concerning zero-initialization of added weights. Zero-initializing $\W_\beta$ will get the overall best results in our experiments.}
\label{tab:more_abla}
\end{table}



==> table_result/params.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[h!]\fontsize{8.5}{9}\selectfont
% \vspace{-0.8em}
\centering
\resizebox{\textwidth}{!}{%
% \begin{tabular}{ccccccccc}
\begin{tabular*}{\hsize}{@{}@{\extracolsep{\fill}}lcccccccc@{}}\midrule
% \midrule
\textbf{} &
  \multicolumn{4}{c}{\textbf{LLaMA}} &
  \multicolumn{3}{c}{\textbf{LLaMA-2}} \\ \midrule
\textbf{} &
  \multicolumn{1}{c}{\text{7B}} &
  \multicolumn{1}{c}{\text{13B}} &
  \multicolumn{1}{c}{\text{30B}} &
  \text{65B} &
  \multicolumn{1}{c}{\text{7B}} &
  \multicolumn{1}{c}{\text{13B}} &
  \text{70B} \\ \midrule
\text{Trainable Parameters} &
  \multicolumn{1}{c}{2.0$\times$10$^7$} &
  \multicolumn{1}{c}{3.1$\times$10$^7$} &
  \multicolumn{1}{c}{6.0$\times$10$^7$} &
  9.8$\times$10$^7$ &
  \multicolumn{1}{c}{2.0$\times$10$^7$} &
  \multicolumn{1}{c}{3.1$\times$10$^7$} &
  1.1$\times$10$^8$ \\ %\midrule
\text{All Parameters} &
  \multicolumn{1}{c}{6.8$\times$10$^9$} &
  \multicolumn{1}{c}{1.3$\times$10$^{10}$} &
  \multicolumn{1}{c}{3.3$\times$10$^{10}$} &
  6.5$\times$10$^{10}$ &
  \multicolumn{1}{c}{6.8$\times$10$^9$} &
  \multicolumn{1}{c}{1.3$\times$10$^{10}$} &
  6.9$\times$10$^{10}$ \\ %\midrule
\textbf{Per mille (\textperthousand)} &
  \multicolumn{1}{c}{\textbf{2.90}} &
  \multicolumn{1}{c}{\textbf{2.35}} &
  \multicolumn{1}{c}{\textbf{1.83}} &
  \textbf{1.50} &
  \multicolumn{1}{c}{\textbf{2.90}} &
  \multicolumn{1}{c}{\textbf{2.35}} &
  \textbf{1.54} \\ \midrule
\end{tabular*}%
}
\vspace{-0.5em}
\caption{Number of trainable parameters, total number of parameters, and per mille of trainable parameters of SPP with $r=16$. We only need to fine-tune a small fraction of parameters compared with full fine-tuning.}
\label{tab:params_number}
% \vspace{-0.5em}
\end{table*}


==> table_result/ppl.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[h!]\fontsize{8.5}{9}\selectfont
\centering
\resizebox{\textwidth}{!}{%
% \begin{tabular}{ccccccccc}
\begin{tabular*}{\hsize}{@{}@{\extracolsep{\fill}}ccccccccc@{}}\midrule
% \begin{tabular}{ccccccccc}
               &                  & \multicolumn{4}{c}{\textbf{LLaMA}} & \multicolumn{3}{c}{\textbf{LLaMA - 2}}       \\\midrule
\textbf{Algorithm}      & \textbf{Sparsity}         & \textbf{7B}    & \textbf{13B}   & \textbf{30B}   & \textbf{65B}   & \textbf{7B}        & \textbf{13B}   & \textbf{70B}   \\\midrule
N/A            & Dense            & 5.68 & 5.09  & 4.10  & 3.53  & 5.12      & 4.57   & 3.12  \\\midrule
SparseGPT      & Unstructured 50\% & 7.21  & 6.21  & 5.32  & 4.60  & 6.52      & 5.62  & 3.99  \\
SparseGPT\textbf{+Ours} & Unstructured 50\% & 7.27  & 6.09  & 5.36  & 4.59 & 6.35      & 5.42  & 3.99   \\
SparseGPT      & 2:4            & 10.87  & 9.09  & 7.20  & 6.20  & 10.06      & 8.12  & 5.37  \\
SparseGPT\textbf{+Ours} & 2:4            & 8.71  & 7.11  & 6.20  & 6.12   & 7.66      & 6.41  & 5.36  \\\midrule
Wanda          & Unstructured 50\% & 7.26    & 6.15  & 5.25  & 4.60  & 6.46       & 5.58  & 3.97  \\
Wanda\textbf{+Ours}     & Unstructured 50\% & 7.28  & 6.10  & 5.26  & 4.59  & 6.26      & 5.41  & 3.97  \\
Wanda          & 2:4            & 11.53  & 9.57  & 6.90  & 6.24  & 11.32      & 8.37  & 5.20  \\
Wanda\textbf{+Ours}     & 2:4            & 8.72  & 7.20  & 6.20  & 5.90  & 7.78      & 6.49  & 5.07 \\\midrule
\end{tabular*}%
}
\caption{Wikitext PPL~\cite{merity2016pointer} comparison of 50\% sparsity models before andafter SPP fine-tuning. After training, the PPL of all models with 2:4 structured sparsity decreased, and the PPL of most unstructured 50\% sparsity models decreased.}
\label{tab:ppl_cmp}
\end{table*}


==> table_result/zero_shot_llama1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[h!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{clccccccccc}
\midrule
\textbf{LLaMA} &
  \textbf{Method} &
  \textbf{Sparsity} &
  \textbf{BoolQ} &
  \textbf{RTE} &
  \textbf{HellaSwag} &
  \textbf{WinoGrande} &
  \textbf{ARC-e} &
  \textbf{ARC-c} &
  \textbf{OBQA} &
  \textbf{Average} \\ \midrule
\multirow{9}{*}{\textbf{7B}}  & None            & Dense            & 75.11 & 66.43 & 56.96 & 69.85 & 75.25 & 41.89 & 34.40 & 59.98 \\ \cmidrule{2-11} 
                              & SparseGPT      & Unstructured 50\% & \gc{73.36} & \gc{57.76} & \gc{51.44} & \gc{68.03} & \gc{70.45} & \gc{36.35} & \gc{28.40} & \gc{55.11} \\ %\cmidrule{2-11} 
                              & SparseGPT\textbf{+SPP} & Unstructured 50\% & 72.84 & 65.70 & 56.40 & 67.88 & 72.35 & 41.04 & 32.80 & \textbf{58.43} \\ %\cmidrule{2-11} 
                              & SparseGPT      & 2:4              & \gc{70.09} & \gc{57.76} & \gc{43.37} & \gc{63.46} & \gc{61.62} & \gc{29.27} & \gc{22.60} & \gc{49.74} \\ %\cmidrule{2-11} 
                              & SparseGPT\textbf{+SPP} & 2:4              & 72.39 & 59.57 & 53.33 & 64.17 & 68.39 & 37.54 & 26.80 & \textbf{54.60} \\ \cmidrule{2-11} 
                              & Wanda          & Unstructured 50\% & \gc{71.01} & \gc{55.23} & \gc{51.90} & \gc{66.22} & \gc{69.36} & \gc{36.95} & \gc{28.60} & \gc{54.18} \\ %\cmidrule{2-11} 
                              & Wanda\textbf{+SPP}     & Unstructured 50\% & 70.86 & 66.06 & 55.92 & 67.64 & 72.81 & 41.64 & 32.00 & \textbf{58.13} \\ %\cmidrule{2-11} 
                              & Wanda          & 2:4              & \gc{69.27} & \gc{51.26} & \gc{42.07} & \gc{62.67} & \gc{60.52} & \gc{27.99} & \gc{24.60} & \gc{48.34} \\ %\cmidrule{2-11} 
                              & Wanda\textbf{+SPP}     & 2:4              & 71.19 & 63.90 & 52.77 & 64.88 & 68.18 & 37.03 & 30.00 & \textbf{55.42} \\ \midrule
\multirow{9}{*}{\textbf{13B}} & None            & Dense            & 77.98 & 70.40 & 59.92 & 72.61 & 77.36 & 46.50 & 33.20 & 62.57 \\ \cmidrule{2-11} 
                              & SparseGPT      & Unstructured 50\% & \gc{76.54} & \gc{62.09} & \gc{54.94} & \gc{71.59} & \gc{72.35} & \gc{41.64} & \gc{32.20} & \gc{58.76} \\ %\cmidrule{2-11} 
                              & SparseGPT\textbf{+SPP} & Unstructured 50\% & 79.20 & 64.62 & 59.27 & 70.32 & 74.83 & 46.59 & 34.60 & \textbf{61.35} \\ %\cmidrule{2-11} 
                              & SparseGPT      & 2:4              & \gc{70.80} & \gc{56.68} & \gc{48.09} & \gc{69.22} & \gc{66.88} & \gc{36.26} & \gc{26.20} & \gc{53.45} \\ %\cmidrule{2-11} 
                              & SparseGPT\textbf{+SPP} & 2:4              & 77.65 & 63.54 & 56.55 & 69.69 & 71.21 & 40.96 & 32.60 & \textbf{58.89} \\ \cmidrule{2-11} 
                              & Wanda          & Unstructured 50\% & \gc{76.27} & \gc{62.82} & \gc{55.78} & \gc{71.98} & \gc{73.32} & \gc{43.77} & \gc{31.80} & \gc{59.39} \\ %\cmidrule{2-11} 
                              & Wanda\textbf{+SPP}     & Unstructured 50\% & 78.29 & 66.43 & 58.88 & 70.32 & 75.59 & 46.93 & 34.40 & \textbf{61.55} \\ %\cmidrule{2-11} 
                              & Wanda          & 2:4              & \gc{70.21} & \gc{53.79} & \gc{46.78} & \gc{68.82} & \gc{65.74} & \gc{33.70} & \gc{26.20} & 52.18 \\ %\cmidrule{2-11} 
                              & Wanda\textbf{+SPP}     & 2:4              & 75.99 & 58.12 & 56.07 & 68.90 & 70.37 & 40.53 & 32.40 & \textbf{57.48} \\ \midrule
\multirow{9}{*}{\textbf{30B}} & None            & Dense            & 82.63 & 66.79 & 63.36 & 75.85 & 80.39 & 52.82 & 36.00 & 65.41 \\ \cmidrule{2-11} 
                              & SparseGPT      & Unstructured 50\% & \gc{82.63} & \gc{58.84} & \gc{59.20} & \gc{73.48} & \gc{78.79} & \gc{49.15} & \gc{33.20} & \gc{62.18} \\ %\cmidrule{2-11} 
                              & SparseGPT\textbf{+SPP} & Unstructured 50\% & 84.43 & 68.23 & 63.18 & 73.56 & 81.57 & 52.56 & 37.00 & \textbf{65.79} \\ %\cmidrule{2-11} 
                              & SparseGPT      & 2:4              & \gc{76.57} & \gc{61.01} & \gc{53.52} & \gc{72.30} & \gc{74.66} & \gc{42.06} & \gc{31.60} & \gc{58.82} \\ %\cmidrule{2-11} 
                              & SparseGPT\textbf{+SPP} & 2:4              & 81.65 & 66.43 & 60.46 & 72.45 & 78.75 & 50.17 & 36.20 & \textbf{63.73} \\ \cmidrule{2-11} 
                              & Wanda          & Unstructured 50\% & \gc{81.93} & \gc{64.98} & \gc{60.95} & \gc{73.64} & \gc{79.38} & \gc{50.17} & \gc{34.80} & \gc{63.69} \\ %\cmidrule{2-11} 
                              & Wanda\textbf{+SPP}     & Unstructured 50\% & 84.19 & 66.79 & 62.52 & 71.59 & 77.10 & 51.79 & 34.80 & \textbf{64.11} \\ %\cmidrule{2-11} 
                              & Wanda          & 2:4              & \gc{75.14} & \gc{63.54} & \gc{54.53} & \gc{72.45} & \gc{74.24} & \gc{41.89} & \gc{31.80} & \gc{59.08} \\ %\cmidrule{2-11} 
                              & Wanda\textbf{+SPP}     & 2:4              & 81.38 & 69.68 & 59.99 & 71.59 & 76.73 & 48.63 & 34.60 & \textbf{63.23} \\ \midrule
\multirow{9}{*}{\textbf{65B}} & None            & Dense            & 84.55 & 69.68 & 65.40 & 77.35 & 52.82 & 81.00 & 38.00 & 66.97 \\ \cmidrule{2-11} 
                              & SparseGPT      & Unstructured 50\% & \gc{84.90} & \gc{70.04} & \gc{63.95} & \gc{77.27} & \gc{79.65} & \gc{50.17} & \gc{37.40} & \gc{66.20} \\ %\cmidrule{2-11} 
                              & SparseGPT\textbf{+SPP} & Unstructured 50\% & 84.95 & 70.04 & 64.25 & 77.19 & 79.85 & 50.94 & 37.80 & \textbf{66.43} \\ %\cmidrule{2-11} 
                              & SparseGPT      & 2:4              & \gc{84.55} & \gc{69.31} & \gc{57.95} & \gc{76.95} & \gc{78.00} & \gc{45.39} & \gc{31.20} & \gc{63.34} \\ %\cmidrule{2-11} 
                              & SparseGPT\textbf{+SPP} & 2:4              & 84.25 & 68.23 & 58.40 & 76.87 & 78.10 & 45.99 & 31.40 & 63.32 \\ \cmidrule{2-11} 
                              & Wanda          & Unstructured 50\% & \gc{85.05} & \gc{71.84} & \gc{64.60} & \gc{77.35} & \gc{79.65} & \gc{50.26} & \gc{38.40} & \gc{66.74} \\ %\cmidrule{2-11} 
                              & Wanda\textbf{+SPP}     & Unstructured 50\% & 85.25 & 71.84 & 65.30 & 77.19 & 79.95 & 51.11 & 38.60 & \textbf{67.03} \\ %\cmidrule{2-11} 
                              & Wanda          & 2:4              & \gc{83.40} & \gc{61.01} & \gc{58.55} & \gc{75.22} & \gc{76.60} & \gc{45.56} & \gc{33.20} &\gc{61.93} \\ %\cmidrule{2-11} 
                              & Wanda\textbf{+SPP}     & 2:4              & 83.30 & 61.37 & 61.85 & 76.16 & 78.60 & 47.70 & 36.20 & \textbf{63.60} \\ \midrule
\end{tabular}%
}
\vspace{-0.5em}
\caption{Zero-shot evaluation results of 7 tasks from EleutherAI LM Harness~\cite{gao2021framework} after training LLaMA on Alpaca~\cite{taori2023alpaca} dataset by SPP. SPP improves the performance of sparse models from SparseGPT and Wanda. In 2 cases, the performance of sparsely trained models even exceeds their dense counterparts.}
\label{tab:zero_llama1_50}
\vspace{-1em}
\end{table*}



==> table_result/zero_shot_llama2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[h!]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{clccccccccc}
\midrule
\textbf{LLaMA - 2} &
  \textbf{Method} &
  \textbf{Sparsity} &
  \textbf{BoolQ} &
  \textbf{RTE} &
  \textbf{HellaSwag} &
  \textbf{WinoGrande} &
  \textbf{ARC-e} &
  \textbf{ARC-c} &
  \textbf{OBQA} &
  \textbf{Average} \\ \midrule
\multirow{9}{*}{\textbf{7B}}  & None            & Dense            & 77.74 & 62.82 & 57.17 & 68.98 & 76.30 & 43.43 & 31.40 & 59.69 \\ \cmidrule{2-11} 
                              & SparseGPT      & Unstructured 50\% & 76.24 & 55.96 & 52.87 & 68.98 & 71.55 & 37.80 & 28.60 & 56.00 \\ %\cmidrule{2-11} 
                              & SparseGPT\textbf{+SPP} & Unstructured 50\% & 75.75 & 56.32 & 55.32 & 69.14 & 74.20 & 42.49 & 30.80 & 57.72 \\ %\cmidrule{2-11} 
                              & SparseGPT      & 2:4              & 66.91 & 57.76 & 43.55 & 66.14 & 64.10 & 31.40 & 24.20 & 50.58 \\ %\cmidrule{2-11} 
                              & SparseGPT\textbf{+SPP} & 2:4              & 70.89 & 54.15 & 51.33 & 67.40 & 70.96 & 38.99 & 29.00 & 54.67 \\ \cmidrule{2-11} 
                              & Wanda          & Unstructured 50\% & 76.73 & 53.43 & 52.50 & 68.43 & 72.35 & 39.16 & 30.80 & 56.20 \\ %\cmidrule{2-11} 
                              & Wanda\textbf{+SPP}     & Unstructured 50\% & 77.31 & 54.15 & 55.19 & 67.96 & 74.96 & 42.24 & 33.00 & 57.83 \\ %\cmidrule{2-11} 
                              & Wanda          & 2:4              & 68.47 & 53.07 & 41.33 & 62.67 & 62.88 & 30.55 & 23.60 & 48.94 \\ %\cmidrule{2-11} 
                              & Wanda\textbf{+SPP}     & 2:4              & 72.91 & 54.51 & 50.61 & 64.48 & 70.71 & 37.88 & 28.60 & 54.24 \\ \midrule
\multirow{9}{*}{\textbf{13B}} & None            & Dense            & 80.55 & 65.34 & 60.04 & 72.14 & 79.42 & 48.46 & 35.20 & 63.02 \\ \cmidrule{2-11} 
                              & SparseGPT      & Unstructured 50\% & 81.93 & 62.45 & 55.83 & 70.88 & 75.13 & 42.49 & 32.40 & 60.16 \\ %\cmidrule{2-11} 
                              & SparseGPT\textbf{+SPP} & Unstructured 50\% & 80.67 & 65.70 & 58.47 & 70.88 & 77.02 & 46.59 & 34.20 & 61.93 \\ %\cmidrule{2-11} 
                              & SparseGPT      & 2:4              & 78.62 & 56.68 & 48.32 & 68.51 & 68.52 & 36.01 & 27.40 & 54.87 \\ %\cmidrule{2-11} 
                              & SparseGPT\textbf{+SPP} & 2:4              & 78.10 & 67.15 & 55.29 & 70.24 & 72.73 & 43.00 & 30.80 & 59.62 \\ \cmidrule{2-11} 
                              & Wanda          & Unstructured 50\% & 81.13 & 58.84 & 57.07 & 70.72 & 75.67 & 42.83 & 32.20 & 59.78 \\ %\cmidrule{2-11} 
                              & Wanda\textbf{+SPP}     & Unstructured 50\% & 80.92 & 69.31 & 58.45 & 71.82 & 78.49 & 46.84 & 34.20 & 62.86 \\ %\cmidrule{2-11} 
                              & Wanda          & 2:4              & 76.09 & 55.96 & 46.19 & 67.56 & 68.64 & 34.13 & 24.20 & 53.25 \\ %\cmidrule{2-11} 
                              & Wanda\textbf{+SPP}     & 2:4              & 76.70 & 66.43 & 55.02 & 68.11 & 72.60 & 42.24 & 31.00 & 58.87 \\ \midrule
\multirow{9}{*}{\textbf{70B}} & None            & Dense            & 83.45 & 67.87 & 66.05 & 77.98 & 82.55 & 54.44 & 37.20 & 67.08 \\ \cmidrule{2-11} 
                              & SparseGPT      & Unstructured 50\% & 84.75 & 71.84 & 64.10 & 78.22 & 81.55 & 52.73 & 37.20 & 67.20 \\ %\cmidrule{2-11} 
                              & SparseGPT\textbf{+SPP} & Unstructured 50\% & 84.75 & 72.20 & 64.05 & 78.06 & 81.65 & 52.73 & 37.20 & 67.23 \\ %\cmidrule{2-11} 
                              & SparseGPT      & 2:4              & 81.30 & 69.31 & 58.60 & 76.24 & 79.50 & 48.21 & 32.60 & 63.68 \\ %\cmidrule{2-11} 
                              & SparseGPT\textbf{+SPP} & 2:4              & 81.30 & 68.59 & 58.80 & 76.24 & 79.40 & 48.29 & 32.60 & 63.60 \\ \cmidrule{2-11} 
                              & Wanda          & Unstructured 50\% & 82.50 & 72.56 & 63.90 & 78.06 & 81.60 & 52.47 & 37.80 & 66.98 \\ %\cmidrule{2-11} 
                              & Wanda\textbf{+SPP}     & Unstructured 50\% & 82.25 & 72.92 & 64.40 & 77.90 & 81.70 & 53.24 & 37.60 & 67.14 \\ %\cmidrule{2-11} 
                              & Wanda          & 2:4              & 79.55 & 67.87 & 59.05 & 76.24 & 79.40 & 47.70 & 35.40 & 63.60 \\ %\cmidrule{2-11} 
                              & Wanda\textbf{+SPP}     & 2:4              & 80.25 & 69.31 & 60.65 & 76.01 & 80.10 & 48.81 & 35.20 & 64.33 \\ \midrule
\end{tabular}%
}
\caption{Zero-shot evaluation of 7 different tasks from EleutherAI LM Harness~\cite{gao2021framework} after training LLaMA-2 on Stanford-Alpaca~\cite{taori2023alpaca} by SPP. As can be seen from the table, SPP can improve the performance of sparse models.}
\label{tab:zero_llama2_50}
\end{table}

